A new physical interpretation of optical and infrared variability in quasars

Changing-look quasars are a recently identified class of active galaxies in which the strong UV continuum and/or broad optical hydrogen emission lines associated with unobscured quasars either appear or disappear on timescales of months to years. The physical processes responsible for this behaviour are still debated, but changes in the black hole accretion rate or accretion disk structure appear more likely than changes in obscuration. Here we report on four epochs of spectroscopy of SDSS J110057.70-005304.5, a quasar at a redshift of $z=0.378$ whose UV continuum and broad hydrogen emission lines have faded, and then returned over the past $\approx$20 years. The change in this quasar was initially identified in the infrared, and an archival spectrum from 2010 shows an intermediate phase of the transition during which the flux below rest-frame $\approx$3400\AA\ has decreased by close to an order of magnitude. This combination is unique compared to previously published examples of changing-look quasars, and is best explained by dramatic changes in the innermost regions of the accretion disk. The optical continuum has been rising since mid-2016, leading to a prediction of a rise in hydrogen emission line flux in the next year. Increases in the infrared flux are beginning to follow, delayed by a $\sim$3 year observed timescale. If our model is confirmed, the physics of changing-look quasars are governed by processes at the innermost stable circular orbit (ISCO) around the black hole, and the structure of the innermost disk. The easily identifiable and monitored changing-look quasars would then provide a new probe and laboratory of the nuclear central engine.

==> Makefile <==

TEXFILE=Ross_etal_J1100_MNRAS_rv1

default: all
# just run it


bib: 
	bibtex ${TEXFILE}

all :
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
	bibtex ${TEXFILE}
	bibtex ${TEXFILE}
	bibtex ${TEXFILE}
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
	rm -f  ${TEXFILE}.aux
#	rm -f  ${TEXFILE}.bbl
	rm -f  ${TEXFILE}.blg
	rm -f  ${TEXFILE}.dvi
	rm -f  ${TEXFILE}.log
	rm -f  ${TEXFILE}.out
	rm -f  ${TEXFILE}.toc
#	rm -f  ${TEXFILE}Notes.bib
	open ${TEXFILE}.pdf


clean:
	rm -f \
	${TEXFILE}.dvi \
	${TEXFILE}.ps \
	${TEXFILE}.out \
	${TEXFILE}.aux \
	${TEXFILE}.bbl \
	${TEXFILE}.blg \
	${TEXFILE}.toc \
	${TEXFILE}.log 
#	${TEXFILE}.pdf 





==> notes4posting <==
https://arxiv.org/user/

Enter Metadata: Title, Authors, Abstract, Comments, etc.
*Title:

A new physical interpretation of optical and infrared variability in quasars

*Author(s): (first names first; do not use et al.; separate with commas or 'and'; see linked help)

Nicholas P. Ross, K. E. Saavik Ford, Matthew Graham, Barry McKernan, Daniel Stern, Aaron M. Meisner, Roberto J. Assef, Arjun Dey, Andrew J. Drake, Hyunsung D. Jun, Dustin Lang


*Abstract:
Changing-look quasars are a recently identified class of active galaxies in which the strong UV continuum and/or broad optical hydrogen emission lines associated with unobscured quasars either appear or disappear on timescales of months to years.  The physical processes responsible for this behaviour are still debated, but changes in the black hole accretion rate or accretion disk structure appear more likely than changes in obscuration. Here we report on four epochs of spectroscopy of SDSS J110057.70-005304.5, a quasar at a redshift of $z=0.378$ whose UV continuum and broad hydrogen emission lines have faded, and then returned over the past $\approx$20 years. The change in this quasar was initially identified in the infrared, and an archival spectrum from 2010 shows an intermediate phase of the transition during which the flux below rest-frame $\approx$3400\AA\ has decreased by close to an order of magnitude. This combination is unique compared to previously published examples of changing-look quasars, and is best explained by dramatic changes in the innermost regions of the accretion disk. The optical continuum has been rising since mid-2016, leading to a prediction of a rise in hydrogen emission line flux in the next year. Increases in the infrared flux are beginning to follow, delayed by a $\sim$3 year observed timescale. If our model is confirmed, the physics of changing-look quasars are governed by processes at the innermost stable circular orbit (ISCO) around the black hole, and the structure of the innermost disk. The easily identifiable and monitored changing-look quasars would then provide a new probe and laboratory of the nuclear central engine.


Comments: (e.g.: 10 pages, 5 figures, conference or other essential info)
13 pages, 4 figures, 3 tables. Published in MNRAS, 2018MNRAS.480.4468R
All code and data links on GitHub, https://github.com/d80b2t/WISE_LC. 

Journal-ref:  2018MNRAS.480.4468R.
DOI: 	      10.1093/mnras/sty2002. 
